A Living Review of Machine Learning for Particle Physics

Modern machine learning techniques, including deep learning, are rapidly being applied, adapted, and developed for high energy physics. Given the fast pace of this research, we have created a living review with the goal of providing a nearly comprehensive list of citations for those developing and applying these approaches to experimental, phenomenological, or theoretical analyses. As a living document, it will be updated as often as possible to incorporate the latest developments. A list of proper (unchanging) reviews can be found within. Papers are grouped into a small set of topics to be as useful as possible. Suggestions and contributions are most welcome, and we provide instructions for participating.

==> Makefile <==
FILENAME = ms

date = $(shell date +%Y-%m-%d)
output_file = draft_$(date).pdf

figure_src = $(wildcard figures/*.tex figures/*/*.tex)
figure_list = $(figure_src:.tex=.pdf)

LATEX = pdf 

BIBTEX = bibtex

default: document copy_draft

all: default

figures: $(figure_list)

figures/%.pdf: figures/%.tex
	latexmk -$(LATEX) -interaction=nonstopmode -halt-on-error $(basename $@)
	mv $(notdir $(basename $@)).pdf $(basename $@).pdf
	rm $(notdir $(basename $@)).*

text:
	latexmk -$(LATEX) -logfilewarnings -halt-on-error -shell-escape $(FILENAME)

document: figures text

copy_draft:
	rsync $(FILENAME).pdf $(output_file)

clean:
	rm -f *.aux *.bbl *.blg *.dvi *.idx *.lof *.log *.lot *.toc \
		*.xdy *.nav *.out *.snm *.vrb *.mp \
		*.synctex.gz *.brf *.fls *.fdb_latexmk \
		*.glg *.gls *.glo *.ist *.alg *.acr *.acn \
		mainNotes.bib

clean_figures:
	rm -f $(figure_list)

clean_drafts:
	rm -f draft_*.pdf

realclean: clean clean_figures
	rm -f *.ps *.pdf

lint:
	grep -E --color=always -r -i --include=\*.tex --include=\*.bib "(\b[a-zA-Z]+) \1\b" || true

final:
	if [ -f *.aux ]; then \
		$(MAKE) clean; \
	fi
	$(MAKE) figures
	$(MAKE) abstract
	$(MAKE) text
	$(MAKE) clean
	$(MAKE) lint

arXiv: realclean document
	mkdir submit_to_arXiv
	cp *.tex submit_to_arXiv
	cp *.bbl submit_to_arXiv/ms.bbl
	cp Makefile submit_to_arXiv
	cp -r figures submit_to_arXiv
	mv submit_to_arXiv/main.tex submit_to_arXiv/ms.tex
	
	
	sed -i.bak '/^ *
	
	sed -i.bak '/{hyperref}/d' submit_to_arXiv/ms.tex
	find submit_to_arXiv/ -name "*.bak" -type f -delete
	
	find submit_to_arXiv/ -name "*.bib" -type f -delete
	tar -zcvf submit_to_arXiv.tar.gz submit_to_arXiv/
	rm -rf submit_to_arXiv
	$(MAKE) realclean

clean_arXiv:
	if [ -f submit_to_arXiv.tar.gz ];then \
		rm submit_to_arXiv.tar.gz; \
	fi

deep_clean: realclean clean_arXiv
	rm -rf submit_to_arXiv

